Development and Justification of a Physical Layer Model Based on Monitoring Data for Quantum Key Distribution

Quantum Key Distribution (QKD) is a promising technique for ensuring long-term security in communication systems. Unlike conventional key exchange methods like RSA, which quantum computers could theoretically break [1], QKD offers enhanced security based on quantum mechanics [2]. Despite its maturity and commercial availability, QKD devices often have undisclosed implementations and are tamper-protected. This thesis addresses the practical imperfections of QKD systems, such as low and fluctuating Secret Key Rates (SKR) and unstable performance. By applying theoretical SKR derivations to measurement data from a QKD system in Poland, we gain insights into current system performance and develop machine learning (ML) models to predict system behavior. Our methodologies include creating a theoretical QKD model [2] and implementing ML models using tools like Keras (TensorFlow [3]). Key findings reveal that while theoretical models offer foundational insights, ML models provide superior accuracy in forecasting QKD system performance, adapting to environmental and operational parameters. This thesis highlights the limitations of theoretical models and underscores the practical relevance of ML models for QKD systems. Future research should focus on developing a comprehensive physical layer model capable of doing long-term forcasting of the SKR. Such a model could prevent an encryption system form running out of keys if the SKR drops significantly. In summary, this thesis establishes a foundational approach for using ML models to predict QKD system performance, paving the way for future advancements in SKR long-term predictions.

==> Formatting.tex <==
\chapter{Formatting}

\section{Figures and Tables}
Figures and tables need to include a caption. This can be done with the LaTeX-command \texttt{\bslash caption$\lbrace\rbrace$}. To be able to reference figures and tables, a \texttt{\bslash label$\lbrace\rbrace$} must follow the caption.

\begin{figure}[h!]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{phd112013s.eps}
    \caption{Ein PHD Comic}
    \label{fig:ToUseWithReference}
  \end{center}
\end{figure}

\begin{table}[b]
\begin{center}
\begin{tabular}{|l |c|}
\hline 
\textbf{Parameter} & \textbf{Value} \\
\hline  
\hline 
Transmission Power & 23~dBm\\
\hline 
Center Frequency & 2.6~GHz\\
\hline 
Channel Bandwidth & 15~kHz\\
\hline 
Shadowing Correlation Distance & 40~m\\
\hline 
Noise Density & -174~dBm/Hz\\
\hline 
Antenna Heights & 1.5~m\\
\hline 
\end{tabular}
\caption{Simulation Parameters and Values}\label{tab:param_table}
\end{center}
\end{table}

The labelled figures and tables can be referenced via \texttt{\bslash ref}, e.g. ~Figure~\ref{fig:ToUseWithReference}.
\newpage

\section{Referencing}
Literature references are included e.g. like this:\\
``..., as shown in \cite{eberspaecher97},, ...'' or ``... there are several approaches \cite{arnaud99,griswold90} ...''
